NARF24: Estimating Articulated Object Structure for Implicit Rendering

Articulated objects and their representations pose a difficult problem for robots. These objects require not only representations of geometry and texture, but also of the various connections and joint parameters that make up each articulation. We propose a method that learns a common Neural Radiance Field (NeRF) representation across a small number of collected scenes. This representation is combined with a parts-based image segmentation to produce an implicit space part localization, from which the connectivity and joint parameters of the articulated object can be estimated, thus enabling configuration-conditioned rendering.

==> sections/problem_statement.tex <==
Given $N$ images across $K$ scenes, $\{P_{k}^{(i)}, i \leq N, k \leq K\}$, each containing the same articulated object, along with each image's pose $X^{(i)}_{k}$, we seek a function $F(x,y,z,k)=(r,g,b,\sigma)$ [$(x,y,z), (r,g,b) \in \mathbb{R}^3$] that, when integrated along epipolar rays via the volumetric rendering equation \cite{kajiya1986rendering}, minimizes the mean-squared-error loss between the rendered image and ground truth: $\mathcal{L}_{MSE}(\hat{P}_{k}^{(i)}) = \big|\big|\hat{P}_{k}^{(i)} - P_{k}^{(i)}\big|\big|_2$.
%$\hat{P}_{k}^{(i)}$ 
